Stackelberg Attacks on Auctions and Blockchain Transaction Fee Mechanisms

We study an auction with $m$ identical items in a context where $n$ agents can arbitrarily commit to strategies. In general, such commitments non-trivially change the equilibria by inducing a metagame of choosing which strategies to commit to. In this model, we demonstrate a strategy that an attacker may commit to that ensures they receive one such item for free, while forcing the remaining agents to enter into a lottery for the remaining items (albeit for free). The attack is thus detrimental to the auctioneer who loses most of their revenue. For various types of auctions that are not too congested, we show that the strategy works as long as the agents have valuations that are somewhat concentrated. In this case, all agents will voluntarily cooperate with the attacker to enter into the lottery, because doing so gives them a chance of receiving a free item that would have otherwise cost an amount commensurate with their valuation. The attack is robust to a large constant fraction of the agents being either oblivious to the attack or having exceptionally high valuations (thus reluctant to enter into the lottery). For these agents, the attacker may coerce them into cooperating by promising them a free item rather than entering in to the lottery. We show that the conditions for the attack to work hold with high probability when (1) the auction is not too congested, and (2) the valuations are sampled i.i.d. from either a uniform distribution or a Pareto distribution. The attack works for first-price auctions, second-price auctions and the transaction fee mechanism EIP-1559 used by the Ethereum blockchain.

==> 1_prelims.tex <==
\section{Preliminaries}
In this section, we establish notation and briefly state some results that we will make use of in later sections. We use $\log x$ to denote the binary logarithm of $x$. We denote by $\exp(\cdot)$ the exponential function with base $e$, unless otherwise stated. A function $f(x)$ is \emph{negligible} if it grows smaller than the inverse of any polynomial, i.e. if for any constant $c$, $f(x) = o\left(x^{-c}\right)$. We denote by $\negl$ a generic negligible function. We denote by $H(p) = -p \lg p - (1-p) \lg(1-p)$, the binary entropy function, defined on $[0,1]$. Note that $H(p) \leq 1$ for every $p\in[0,1]$. The following bound will be useful later.
\begin{equation}\label{eq:binom_entropy_bound}
    \frac{1}{n+1} 2^{nH(k/n)} \leq {n \choose k} \leq 2^{nH(k/n)}
\end{equation}
\noindent We also note the following upper bound, which will prove useful.
\begin{equation}\label{eq:entropy_upper_bound}
    H(x) \leq 2 \sqrt{x\,(1-x)}
\end{equation}
\noindent We denote by $U(0,1)$ the uniform distribution on $[0,1]$.  Similarly, we define the Pareto distribution with parameter $p>0$ by giving its density function $f$.
\begin{align*}
    f(x) = px^{-p-1} && \text{for $x \geq 1$}.
\end{align*}
We define the Beta distribution $\text{Beta}(\alpha,\beta)$ with parameters $\alpha>0, \beta>0$ as follows.
\begin{align*}
    f(x) = \frac{\Gamma(\alpha+\beta)}{\Gamma(\alpha) \Gamma(\beta)} x^{\alpha-1} (1-x)^{\beta-1}
\end{align*}
where $\Gamma(\cdot)$ is the Gamma function. We will make use of the following concentration bound.
\begin{lemma}[Skorski, \cite{beta_bounds}]\label{lemma:beta_bound}
    Let $X \sim \text{Beta}(\alpha,\beta)$ for $\alpha,\beta>0$, and define,
    \begin{align*}
        v^2 &= \frac{\alpha\beta}{(\alpha+\beta)^2(\alpha+\beta+2)},\\
        c_0 &= \frac{|\beta-\alpha|}{(\alpha+\beta)(\alpha+\beta+2)}\\
        c &= \max\left\{v, c_0 \right\}.
    \end{align*}
    Then for any $\varepsilon>0$, it holds that,
    \begin{align*}
        \Pr\left[X-\E[X] > \varepsilon\right] &\leq \exp\left(-\frac{\varepsilon^2}{2v^2+2c\varepsilon}\right),\\
        \Pr\left[\E[X]-X > \varepsilon\right] &\leq \exp\left(-\frac{\varepsilon^2}{2v^2+2c\varepsilon}\right),
    \end{align*}
\end{lemma}
\subsection{Order Statistics}
Given $n$ i.i.d. samples $X_1, X_2, \ldots, X_n$ from some distribution, we denote by $X_{(1)} < X_{(2)} < \cdots < X_{(n)}$ the $n$ order statistics. When $X_1, X_2, \ldots, X_n \sim U[0,1]$ are sampled i.i.d. from a uniform distribution, we have that 
\begin{equation}\label{order_stats_beta_distr}
    X_{(i)} \sim \text{Beta}(i, n+1-i)
\end{equation}
Note that the order statistics are highly correlated. The expectation of a Beta distribution $\text{Beta}(\alpha, \beta)$ is $\mathbb{E}(X)=\frac{\alpha}{\alpha + \beta}$ and the variance is $\text{Var}[X]= \frac{\alpha \beta}{(\alpha+\beta)^2(\alpha + \beta+1)}$. Later, we will be interested in the quantity $X_{(j)} / X_{(i)}$ for $i<j$, where each $X_{(i)}$ is sampled from a uniform distribution, the density function is known as follows.
\begin{lemma}[Xu, Mei, Miao, \cite{ratio_order_stats}]\label{lemma:ratio_order_stats}
    Let $X_1, X_2, \ldots, X_n \sim U(0,1)$ be i.i.d. Let $i<j$ and define $R_{ij} = \frac{X_{(j)}}{X_{(i)}}$ and let $f(\cdot)$ be its density function with support $[1,\infty)$. Then for every $r\geq 1$,
    \begin{align*}
        f(r) &
        = \frac{n!(r-1)^{j-i-1}}{(i-1)!(j-i-1)!(n-j)!r^j} \,  \int_{0}^1 (1-u)^{j-1}\,u^{n-j} \, \mathrm{d}u
    \end{align*}
\end{lemma}
A similar result exists when the variables are sampled from a Pareto distribution.
\begin{lemma}[Adler, \cite{pareto_ratio_order}]\label{lemma:pareto_order_stats}
    Let $X_1,X_2, \ldots X_n$ be i.i.d. Pareto distributed with parameter $p>0$. Let $i<j$ and define $R_{ij} = \frac{X_{(j)}}{X_{(i)}}$ and let $f(\cdot)$ be its density function with support $[1,\infty)$. Then for every $r\geq 1$,
    \begin{align*}
        f(r) = \frac{p(n-i)!}{(j-i-1)!(n-j)!} \left(1-\frac{1}{r^p}\right)^{j-i-1} \frac{1}{r^{p(n-j+1)+1}}.
    \end{align*} 
\end{lemma}

We will make use of the following concentration bound on order statistics from the uniform distribution.
\begin{lemma}\label{lemma:bound}
    Let $X_1, X_2, \ldots, X_n \sim U[0,1]$, and let $X_{(1)} < X_{(2)} < \cdots < X_{(n)}$ be the $n$ order statistics. Then, 
    \begin{align*}
        \left \lvert X_{(i)} - \frac{i}{n+1} \right \rvert = \Tilde{O}(1/n), && \text{for every $i=1\ldots n$},
    \end{align*}
    except with negligible probability in $n$.
\end{lemma}

\begin{proof}
    We make use of \cref{lemma:beta_bound} to bound the error term and must therefore first find the relevant values of $v$ and $c_0$.  It is a fact that such order statistics have the distribution $\text{Beta}(i, n+1-i)$, i.e. $\alpha = i$ and $\beta = n+1-i$. Thus, for all values of $i$, we must have $\alpha + \beta = n+1$.  It is easy to see that we find the largest value $v^2$ from \cref{lemma:beta_bound} when $\alpha = \beta = \frac{n+1}{2}$.  This case yields 
\begin{align*}
    v^2 \leq \frac{\frac{n+1}{2}\frac{n+1}{2}}{\left(\frac{n+1}{2}+\frac{n+1}{2}\right)^2\left(\frac{n+1}{2}+\frac{n+1}{2}+2\right)}=\frac{1}{4(n+3)}.
\end{align*}
The value of $c_0$ is largest when the numerator is largest, which is clearly when $|\beta - \alpha| = n-1$. Note that this is a specifically different case from when $v^2$ is largest.  When we go on to find the error bounds on specific $v_i$'s we will refine the bound at this step. Thus, we have the following bounding value 
\begin{align*}
    c_0 \leq \frac{n-1}{(n+1)(n+3)}
\end{align*}
It is easy to see that $c = \max \{v, c_0 \}=c_0$.
Thus we can write down the bound for any $i$,
\begin{align*}
     \Pr\left[\left\lvert X_{(i)} - \E[X_{(i)}]\right\rvert > \delta\right] 
        &< 2\exp\left(-\frac{\delta^2}{2v^2+2c\delta}\right)\\
        &\leq 2\exp\left(-\frac{\delta^2}{2\frac{1}{4(n+3)}+\frac{2\delta(n-1)}{(n+1)(n+3)}}\right)\\
        &= 2\exp\left(-\frac{\delta^22(n+3)(n+1)}{(n+1)+4\delta(n-1)}\right)\\
        &< 2\exp\left(-\frac{\delta^2 2n^2}{(n+1)+4\delta n}\right)\\
        &\approx 2\exp\left(-\frac{\delta^2 2n}{1+4\delta }\right)\\
        &=2 \exp (-\Omega (\delta n)).
\end{align*}
If we take $\delta=\frac{\log^2{n}}{n+1}=\Tilde{O}(1/n)$, we obtain the bound, 
\begin{align}
     \Pr\left[\left\lvert X_{(i)} - \E[X_{(i)}]\right\rvert > \delta\right] < 2 \exp(-\omega(\log n)),
\end{align}
which is negligible in $n$. We conclude by doing a union bound on all $n$ valuations. 
\end{proof}

\subsection{Game Theory}
We give a brief recap of game theory to establish notation; refer to \cite{osborne} for more details. An $n$-player game $G$ in extensive form consists of a tree $T$ whose branches are partitioned into $n$ sets, one belonging to each player. We say a branch is owned by a player if it belongs to their partition. Each leaf $\ell$ of the game is labeled with a utility vector $u(\ell) \in \mathbb{R}^n$, denoting the utility given to each player when the game terminates in $\ell$. We denote by $L$ the set of leaves in $G$. The game is played, starting at the root, recursively letting the player who owns the current node choose a subgame to recurse into. A mapping $s_i$ that determines the moves for a player is called a strategy. A set of strategies, one for each player, is called a strategy profile $s$ and determines a distribution on the leafs. We overload notation and denote by $u_i(s)$ the expected utility of parties when employing the strategy profile $s$. This definition suffices for games of perfect information, though more generally we may consider partitioning each players set of branches into information sets. The mapping is then given as input the set to which the current node belongs. The parties are assumed to be rational, risk-neutral, and have quasilinear utilities. We assume parties are weakly malicious, that is, when given multiple options with the same utility, they prefer outcomes with worse utilities for the other players. A strategy profile $s^*$ is said to be an \emph{equilibrium} if for every $i$, and every $s_i$, it holds that $u_i(s_i^*, s_{-i}^*) \geq u_i(s_i, s_{-i}^*)$. If this holds at every subgame, we say $s^*$ is a \emph{subgame perfect equilibrium} (SPE). If, in addition, all such inequalities are strict with a gap of size $\varepsilon\geq 0$, we say the strategy profile $s^*$ has \emph{$\varepsilon$-strong game-theoretic security}. Following the definition of \cite{good_contract}, a strategy profile $s^*$ has \emph{$\varepsilon$-strong game-theoretic security} if, for any $i \in [n]$ and any $s_i \neq s_i^*$, it holds that,
    $$
        u_i(s_i^*, s_{-i}^*) \geq u_i(s_i, s_{-i}^*) + \varepsilon.
    $$ 
With slight overload of notation, we say that a game $G$ with an implicit \emph{intended strategy profile} $s^*$ enjoys $\varepsilon$-strong game-theoretic security if $s^*$ has $\varepsilon$-strong game-theoretic security in $G$. For decentralized commerce, the intended strategy profile is for the seller and buyer to act honestly.  We define the social welfare of a strategy profile $s$ to be $\text{Welf}(s) = \sum_{i=1}^n u_i(s)$.  

Let $G$ be a game with set of strategy profiles $S$. We call a strategy profile $s^*$ a \emph{social optimum} if $\text{Welf}(s^*) = \max_{s \in S} \text{Welf}(s)$ We denote by $E \subseteq S$ the set of equilibria, which is guaranteed to be non-empty. We define the \emph{price of anarchy} as the ratio of social welfare between the social optimum and the worst equilibrium \cite{poa}. 
\begin{equation}\label{eq:poa}
    PoA = \frac{\max_{s \in S}\text{Welf}(s)}{\min_{s \in E} \text{Welf}(s)}
\end{equation}
The price of anarchy measures the inefficiency of a game, with larger values corresponding to more inefficient games.

We are interested in a slightly different measure where we compare the existing SPE without contracts to the equilibria with contracts.  The contract equilibria do not constitute the social optimal, but do allow for relatively more organization as compared to the unorganized case.  The original idea of PoA arose from a need to articulate the difference between unorganized and perfectly optimized systems. Our needs are for a similar mechanism of comparison, but without considering the absolute best outcome.

Taking queues from the existing concept of Price of Anarchy, we define the Price of Defiance, a more general ratio of sets of equilibrium. Take two sets $C \subseteq S$, some set of strategies, and $E \subseteq S$ the set of equilibria of the game, as above. We take the set $C$ to be the set of equilibria after a successful contract attack has been deployed. Define
\begin{equation}\label{eq:pod}
    PoD = \frac{\max_{s \in C}\text{Welf}(s)}{\min_{s \in E} \text{Welf}(s)}
\end{equation}
Now, instead of looking at the ratio between  the best possible outcome and the worst equilibrium, we look at the ratio between the best of a subset of possible outcomes and that same worst equilibrium. This differs from the PoA in that we want to compare some subset of strategies, here those that become equilibria due to the introduction of a contract attack, rather the optimal solution, to the game's usual equilibria. We have  PoD $\leq$ PoA. 

\subsection{Blockchains and Transaction Mechanisms}
Blockchains are decentralized stores of data that consist of blocks that are linked together using cryptographic hash functions. The blocks are generated by a decentralized set of miners who intermittently publish new blocks. The rate of new blocks is controlled by forcing the miners to solve a hard cryptographic puzzle to produce a valid block\footnote{Such blockchains are known as \emph{proof-of-work} (PoW) and require the miners to expend a significant amount of energy. An alternative implementation uses the stake by the miners and are known as \emph{proof-of-stake} (PoS) blockchains \cite{king2012ppcoin,saleh2021blockchain}.}, such that in expectation one block is produced every intended time period, e.g. 12 seconds for Ethereum. Each block has a limited amount of space, which means that, during periods of high congestion, the miners must choose which data to include in the next block. One natural transaction mechanism, which is used by Bitcoin, is to attach tips to the data.  These tips are paid directly to the miners for including the tipper's data in the next block. This implements a first-price auction where the miner chooses the data with the largest associated tips. However, this is not without its share of problems. For example, it means that all the volatility in the demand is transferred to the size of the tips. This makes it difficult for users to estimate the tip needed. The first-price auction was used by Ethereum, which recently switched to another mechanism, known as EIP-1559. EIP-1559 is a modification of a first-price auction where the bids include a base fee $B>0$ that is burned. The base fee is set such that in expectation, half the capacity of a block is used. It is determined by the network and is increased if the last block was congested and decreased if less than half the space was used. 

\begin{algorithm}\hspace{-1mm}\textsc{\textup{(EIP-1559)}}.\label{alg:eip-1559}
\begin{enumerate}
    \item[1.] Each party $i\in[n]$ submits a transaction of value $v_i>0$ and makes a deposit of $B+\tau_i$ funds where $\tau_i\geq0$ is an optional tip.
    \item[2.] A miner finds a block, and selects a $T\subseteq [n]$ with $|T|=m$ that maximizes $\sum_{i \in T} \tau_i$. If there are multiple such $T$'s, it selects $T$ uniformly at random from all suitable sets.
    \item[3.] Each party $i \in T$ has their transactions included in the block and loses their deposit, in total gaining $v_i - B - \tau_i$ money; each party $j\not\in T$ is returned their deposit of $B+\tau_j$ money and gains 0.
    \item[4.] The miner receives $\sum_{i \in T} \tau_i$ money.
    \item[5.] The network adjusts the base fee $B$ depending on $m$ and $n$.
\end{enumerate}
\end{algorithm}


\subsection{Smart Contracts}
In this section, we will formalize our model of smart contracts. As mentioned, smart contracts are programs run on a virtual machine implemented by a blockchain. Formally, a smart contract is a special type of node with fanout 1 that allows an agent to commit to a strategy in its subgame. Such nodes are syntactic sugar for a larger tree that contains a node owned by the contract player with a subgame for each contract they can deploy. For multiple nodes, the contracts are expanded in a bottom-up manner. This model was studied by Hall-Andersen and Schwartzbach, who show that such games constitute a hierarchy that includes Stackelberg games \cite{stackelberg} and reverse Stackelberg games \cite{reverse_stackelberg,reverse_stackelberg_2} as special cases, respectively games with exactly one or two such nodes. As a result, computing equilibria in such games is hard in the general case, although an efficient algorithm is known for two-player games of perfect information.
\begin{thm}[Hall-Andersen, Schwartzbach, \cite{smart_contracts}]\label{thm:pspace}
    Computing the SPE in games with smart contracts is \PSPACE-hard in general, even for games of perfect information. However, there is a quadratic-time algorithm that computes the SPE in two-contract games of perfect information. 
\end{thm}

We restate the algorithm, simplified to work only on two-player games, for self-containment. Let player 1 have the first contract, and player 2 the the second. Let $A,B \subseteq \mathbb{R}$ and define,
$$
    \textsf{threaten}(A,B) = \{x \in A \mid \exists y \in B. \, y_2 < x_2\}.
$$
as the set of nodes from $A$ that player 1 can threaten player 2 into accepting, using threats from $B$. The algorithm, which we will call Algorithm 1, computes the set of nodes that are inducible by a contract for the first player (the inducible region \cite{inducibleregion}) and selects the node that maximizes their utility. For simplicity, assume $G$ is a bifurcating tree. The algorithm recursively computes the nodes that player 1 can induce in the left and right subtrees and combines them at each branch.

\begin{algorithm}\hspace{-1.125mm}\textsc{\textup{(Hall-Andersen, Schwartzbach, \cite{smart_contracts})}}.\\[2mm]$\textsf{InducibleRegion}(G):$
\begin{enumerate}
    \item[1.] If $G$ is a leaf $\ell$, stop and return $\{\ell\}$.
    \item[2.] If $G$ is a node owned by $i$, with children $G^L$ and $G^R$:
    \begin{enumerate}
        \item[] $I^L \gets \textsf{InducibleRegion}(G^L)$.
        \item[] $I^R \gets \textsf{InducibleRegion}(G^R)$.
        \item[] If $i=1$:
        \begin{enumerate}
            \item[] return $I^L \cup I^R \cup \textsf{threaten}(L, I^L \cup I^R)$.
        \end{enumerate}
        \item[] If $i=2$:
        \begin{enumerate}
            \item[] return $\textsf{threaten}(I^R, I^L)\cup\textsf{threaten}(I^L,I^R)$.
        \end{enumerate}
    \end{enumerate}
\end{enumerate}
\end{algorithm}
In practice, running a smart contract requires submitting multiple queries to the blockchain which requires work by the miners and is not free. For the purposes of this work, however, we regard transaction fees as negligible such that we may disregard them entirely. This holds true if the valuations are large compared to the transaction fees. 

==> 2_contracts.tex <==
\section{Side Contract Resilient Auctions}
\begin{itemize}
    \item Tailor the definition to auctions
    \item Remove downward transitivity
    \item Merge it with Section 3
\end{itemize}

\label{sec:resilience}
In this section, we give our definition of games that are resilient to side contract attacks. We show that reasoning about such games is hard in general, but feasible for two-player games of perfect information. We then analyze two decentralized commerce games from the literature and find only one of them is resilient to side contract attacks.

Let $G$ be an extensive-form game on $n$ players. We define $\C_i(G)$ as the game that starts with a smart contract move for player $i$ whose only subgame is $G$. Similarly, if $P : [m] \rightarrow [n]$ is a list of players of length $m$ that specifies the order of the contracts, we denote by $\C_P(G)$ the game with $m$ contracts belonging to the players specified by the list. Generally speaking, being the first player to deploy a smart contract is an advantage.  As a result, the equilibrium of the game may be sensitive to the order of the players in a given list. We call the player with the first contract, $P(1)$, the \emph{leading contract player}. In practice, the order of the players is determined by the consensus protocol used by the underlying blockchain and may be non-deterministic. For the purposes of this paper, we assume the consensus protocol is agnostic to the players and the order is random. Thus, we say a game is side contract resilient if and only if the equilibrium remains the same for any order of the contracts. We will now make this notion more formal.

Let $G, G'$ be two games on $n$ players. We say that $G$ and $G'$ are \emph{equivalent}, written $G \cong G'$, if for every equilibrium $s^*$ in $G$ (respectively, in $G'$) there exists an equilibrium ${s^*}'$ in $G'$ (respectively, in $G$) such that $u_i(s^*) = u_i({s^*}')$ for every $i\in[n]$. Note that this is an equivalence relation.  For two equivalent games, for each equilibrium in either game, there is equilibrium in the other game with the same payoffs. This implicitly means that we regard any two outcomes with the same utility vector as equivalent. While this is not necessarily the case in general, it will be the case for the types of games we consider. Namely, in our case we would have $G$ as an extensive-form game in generic form, meaning that all its utility vectors are distinct, and $G'=\C_P(G)$ the same game with contracts in the order specified by $P$. In the game $G'$, we will have multiple copies of each utility vector from $G$, however all its appearances represent the `same' underlying leaf from the game $G$. 

\begin{definition}[Side Contract Resilience]
    A game $G$ is said to be \emph{side contract $k$-resilient} for an integer $k>0$ if, for any list $P$ of $k$ distinct players, it holds that $\C_P(G) \cong G$. We say $G$ is \emph{(full) side contract resilient} if it is side contract $n$-resilient.
\end{definition} 

If the SPE of a game is unique and labeled with some utility vector $u \in \mathbb{R}^n$, then side-contract resilience says that every SPE in the expanded tree also has to be labeled with $u$.

Note that in this definition, we require the list $P$ to consist of distinct players (i.e. $P$ is injective). If this were not the case, $(k+1)$-resilience would trivially imply $k$-resilience for the uninteresting reason that adding contracts for a fixed player is an idempotent operation, i.e. the same player having two nested contracts is equivalent to them having only the topmost contract. Also note that if a game is not side contract resilient, there exists a side contract that some player can deploy to obtain better utility (or force worse utility for others) as compared to the situation without contracts. Only side contract resilient games are not susceptible to side contract attacks. We observe that side contract resilience does exhibit some form of downward transitivity. We give the case of $1$-resilience from $2$-resilience here (proof is in the appendix). It is unknown if in general $(k+1)$-resilience implies $k$-resilience.

\begin{thm}\label{thm:downward_transitive}
  If a game $G$ is side contract 2-resilient, it is also side contract 1-resilient.
\end{thm}
In general, as observed by \cite{good_contract}, it is hard to reason about side contract resilience. In fact, it follows from the reduction that even determining 1-resilience is $\NP$-hard. However, there is an algorithm for determining 2-resilience for the special case of games with perfect information.


